Using Access Data for Paper Recommendations on ArXiv.org

This thesis investigates in the use of access log data as a source of information for identifying related scientific papers. This is done for arXiv.org, the authority for publication of e-prints in several fields of physics. Compared to citation information, access logs have the advantage of being immediately available, without manual or automatic extraction of the citation graph. Because of that, a main focus is on the question, how far user behavior can serve as a replacement for explicit meta-data, which potentially might be expensive or completely unavailable. Therefore, we compare access, content, and citation-based measures of relatedness on different recommendation tasks. As a final result, an online recommendation system has been built that can help scientists to find further relevant literature, without having to search for them actively.

==> prelim/vita.tex <==
%
% Biographical sketch
%

\begin{biosketch}
Stefan Pohl was born June 21, 1979, in Uecker\"unde, Germany. While attending primary school, he participated in several math competitions.
In 1998 he graduated from Kopernikus--Gymnasium Torgelow with first-class honors and accolade.
\
From 1999 he enrolled as computer science major at University of Applied Sciences, Mittweida Germany.
Beside studies, an internship in a data mining department and vacation work lead to voluntary writing of two accepted and vindicated papers on time series and distributed programming. \todo{In logistic support of run--events (e.g.~marathon), he made an additional commitment.}
In 2004, he was honored for the best overall achievement in studies in conjunction with an outstanding diploma thesis.
\
Later that year, he was admitted as one of the first master's students in computer science with a minor in business management at the Technical University Darmstadt, Germany.
Regardless the additional qualifying exams imposed, he completed all courses with outstanding results and in record time, and even so he found time for an international internship.
\
For his master's thesis, he seized the opportunity to work with Thorsten Joachims at Cornell University, Ithaca, New York on recommendation of citations for the arXiv, probably the largest and most complete scientific preprint collection for physics.
On the basis of his master's thesis, he has written a paper ``Recommending Related Papers Based on Digital Library Access Records'' that has been accepted for JCDL'07.
\end{biosketch}

